Position-Based Multiple-Play Bandits with Thompson Sampling

Multiple-play bandits aim at displaying relevant items at relevant positions on a web page. We introduce a new bandit-based algorithm, PB-MHB, for online recommender systems which uses the Thompson sampling framework. This algorithm handles a display setting governed by the position-based model. Our sampling method does not require as input the probability of a user to look at a given position in the web page which is, in practice, very difficult to obtain. Experiments on simulated and real datasets show that our method, with fewer prior information, deliver better recommendations than state-of-the-art algorithms.

==> PositionBased MultiplePlay Bandits with Thompson Sampling/macros_math.tex <==
\RequirePackage{amsmath, amssymb, mathrsfs, bm, dsfont}

\newcommand{\vect}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\av}{\vect{a}}
\newcommand{\bv}{\vect{b}}
\newcommand{\cv}{\vect{c}}
\newcommand{\dv}{\vect{d}}
\newcommand{\ev}{\vect{e}}
\newcommand{\fv}{\vect{f}}
\newcommand{\gv}{\vect{g}}
\newcommand{\hv}{\vect{h}}
\newcommand{\iv}{\vect{i}}
\newcommand{\jv}{\vect{j}}
\newcommand{\kv}{\vect{k}}
\newcommand{\lv}{\vect{l}}
\newcommand{\mv}{\vect{m}}
\newcommand{\nv}{\vect{n}}
\newcommand{\ov}{\vect{o}}
\newcommand{\pv}{\vect{p}}
\newcommand{\qv}{\vect{q}}
\newcommand{\rv}{\vect{r}}
\newcommand{\sv}{\vect{s}}
\newcommand{\tv}{\vect{t}}
\newcommand{\uv}{\vect{u}}
\newcommand{\vv}{\vect{v}}
\newcommand{\wv}{\vect{w}}
\newcommand{\xv}{\vect{x}}
\newcommand{\yv}{\vect{y}}
\newcommand{\zv}{\vect{z}}
\newcommand{\ellv}{\vect{\ell}}

\newcommand{\onev}{{\pmb{1}}}
\newcommand{\alphav}{{\pmb{\alpha}}}
\newcommand{\betav}{{\pmb{\beta}}}
\newcommand{\gammav}{{\pmb{\gamma}}}
\newcommand{\kappav}{{\pmb{\kappa}}}
\newcommand{\xiv }{{\pmb{\xi}}}
\newcommand{\muv}{{\pmb{\mu}}}
\newcommand{\sigmav}{{\pmb{\sigma}}}
\newcommand{\tauv}{{\pmb{\tau}}}
\newcommand{\thetav}{{\pmb{\theta}}}
\newcommand{\omegav}{{\pmb{\omega}}}
\newcommand{\zetav}{{\pmb{\zeta}}}



\newcommand{\mat}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\Am}{\mat{A}}
\newcommand{\Bm}{\mat{B}}
\newcommand{\Cm}{\mat{C}}
\newcommand{\Dm}{\mat{D}}
\newcommand{\Em}{\mat{E}}
\newcommand{\Fm}{\mat{F}}
\newcommand{\Gm}{\mat{G}}
\newcommand{\Hm}{\mat{H}}
\newcommand{\Imat}{\mat{I}}
\newcommand{\Jm}{\mat{J}}
\newcommand{\Km}{\mat{K}}
\newcommand{\Lm}{\mat{L}}
\newcommand{\Mm}{\mat{M}}
\newcommand{\Nm}{\mat{N}}
\newcommand{\Om}{\mat{O}}
\newcommand{\Pm}{\mat{P}}
\newcommand{\Qm}{\mat{Q}}
\newcommand{\Rm}{\mat{R}}
\newcommand{\Sm}{\mat{S}}
\newcommand{\Tm}{\mat{T}}
\newcommand{\Um}{\mat{U}}
\newcommand{\Vm}{\mat{V}}
\newcommand{\Wm}{\mat{W}}
\newcommand{\Xm}{\mat{X}}
\newcommand{\Ym}{\mat{Y}}
\newcommand{\Zm}{\mat{Z}}
\newcommand{\zerom}{\mat{0}}

\newcommand{\Deltam}{{\mbox{\boldmath$\Delta$}}}
\newcommand{\Gammam}{{\mbox{\boldmath$\Gamma$}}}
\newcommand{\Omegam}{{\mbox{\boldmath$\varOmega$}}}
\newcommand{\Lambdam}{{\mbox{\boldmath$\Lambda$}}}
\newcommand{\Sigmam}{{\mbox{\boldmath$\varSigma$}}}
\newcommand{\Phim}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\Pim}{{\mbox{\boldmath$\Pi$}}}
\newcommand{\Thetam}{{\mbox{\boldmath$\varTheta$}}}




\newcommand{\Ac}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Hc}{{\cal H}}

\newcommand{\RR}{\mathds{R}} %real numbers
\newcommand{\NN}{\mathds{N}} %natural numbers
\newcommand{\CC}{\mathds{C}} %complex numbers
\newcommand{\QQ}{\mathds{Q}} % rational numbers
\newcommand{\EE}{\mathds{E}} %expectation
\newcommand{\PP}{\mathds{P}} % proba
\newcommand{\OO}{{\cal O}} % grand O pour complexité
\newcommand{\ind}{\mathds{1}} % indicatrice




\DeclareMathOperator*{\diag}{\mbox{diag}}
\DeclareMathOperator*{\tr}{\mbox{tr}}
\DeclareMathOperator*{\card}{\mbox{card}}
\DeclareMathOperator*{\cov}{\mbox{cov}}
\DeclareMathOperator*{\sign}{\mbox{sign}}
\DeclareMathOperator*{\var}{\mbox{var}}
%\DeclareMathOperator*{\st}{\mbox{s.t.}}
\DeclareMathOperator*{\rank}{\mbox{rank}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\moyenne}{average}

\DeclareMathOperator*{\Ber}{Ber}
\DeclareMathOperator*{\Beta}{Beta}
\newcommand{\Norm}{{\cal N}}
\DeclareMathOperator*{\sigmoid}{sigmoid}
\DeclareMathOperator*{\logit}{logit}


==> macros_math.tex <==
\RequirePackage{amsmath, amssymb, mathrsfs, bm, dsfont}

\newcommand{\vect}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\av}{\vect{a}}
\newcommand{\bv}{\vect{b}}
\newcommand{\cv}{\vect{c}}
\newcommand{\dv}{\vect{d}}
\newcommand{\ev}{\vect{e}}
\newcommand{\fv}{\vect{f}}
\newcommand{\gv}{\vect{g}}
\newcommand{\hv}{\vect{h}}
\newcommand{\iv}{\vect{i}}
\newcommand{\jv}{\vect{j}}
\newcommand{\kv}{\vect{k}}
\newcommand{\lv}{\vect{l}}
\newcommand{\mv}{\vect{m}}
\newcommand{\nv}{\vect{n}}
\newcommand{\ov}{\vect{o}}
\newcommand{\pv}{\vect{p}}
\newcommand{\qv}{\vect{q}}
\newcommand{\rv}{\vect{r}}
\newcommand{\sv}{\vect{s}}
\newcommand{\tv}{\vect{t}}
\newcommand{\uv}{\vect{u}}
\newcommand{\vv}{\vect{v}}
\newcommand{\wv}{\vect{w}}
\newcommand{\xv}{\vect{x}}
\newcommand{\yv}{\vect{y}}
\newcommand{\zv}{\vect{z}}
\newcommand{\ellv}{\vect{\ell}}

\newcommand{\onev}{{\pmb{1}}}
\newcommand{\alphav}{{\pmb{\alpha}}}
\newcommand{\betav}{{\pmb{\beta}}}
\newcommand{\gammav}{{\pmb{\gamma}}}
\newcommand{\kappav}{{\pmb{\kappa}}}
\newcommand{\xiv }{{\pmb{\xi}}}
\newcommand{\muv}{{\pmb{\mu}}}
\newcommand{\sigmav}{{\pmb{\sigma}}}
\newcommand{\tauv}{{\pmb{\tau}}}
\newcommand{\thetav}{{\pmb{\theta}}}
\newcommand{\omegav}{{\pmb{\omega}}}
\newcommand{\zetav}{{\pmb{\zeta}}}



\newcommand{\mat}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\Am}{\mat{A}}
\newcommand{\Bm}{\mat{B}}
\newcommand{\Cm}{\mat{C}}
\newcommand{\Dm}{\mat{D}}
\newcommand{\Em}{\mat{E}}
\newcommand{\Fm}{\mat{F}}
\newcommand{\Gm}{\mat{G}}
\newcommand{\Hm}{\mat{H}}
\newcommand{\Imat}{\mat{I}}
\newcommand{\Jm}{\mat{J}}
\newcommand{\Km}{\mat{K}}
\newcommand{\Lm}{\mat{L}}
\newcommand{\Mm}{\mat{M}}
\newcommand{\Nm}{\mat{N}}
\newcommand{\Om}{\mat{O}}
\newcommand{\Pm}{\mat{P}}
\newcommand{\Qm}{\mat{Q}}
\newcommand{\Rm}{\mat{R}}
\newcommand{\Sm}{\mat{S}}
\newcommand{\Tm}{\mat{T}}
\newcommand{\Um}{\mat{U}}
\newcommand{\Vm}{\mat{V}}
\newcommand{\Wm}{\mat{W}}
\newcommand{\Xm}{\mat{X}}
\newcommand{\Ym}{\mat{Y}}
\newcommand{\Zm}{\mat{Z}}
\newcommand{\zerom}{\mat{0}}

\newcommand{\Deltam}{{\mbox{\boldmath$\Delta$}}}
\newcommand{\Gammam}{{\mbox{\boldmath$\Gamma$}}}
\newcommand{\Omegam}{{\mbox{\boldmath$\varOmega$}}}
\newcommand{\Lambdam}{{\mbox{\boldmath$\Lambda$}}}
\newcommand{\Sigmam}{{\mbox{\boldmath$\varSigma$}}}
\newcommand{\Phim}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\Pim}{{\mbox{\boldmath$\Pi$}}}
\newcommand{\Thetam}{{\mbox{\boldmath$\varTheta$}}}




\newcommand{\Ac}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Hc}{{\cal H}}

\newcommand{\RR}{\mathds{R}} %real numbers
\newcommand{\NN}{\mathds{N}} %natural numbers
\newcommand{\CC}{\mathds{C}} %complex numbers
\newcommand{\QQ}{\mathds{Q}} % rational numbers
\newcommand{\EE}{\mathds{E}} %expectation
\newcommand{\PP}{\mathds{P}} % proba
\newcommand{\OO}{{\cal O}} % grand O pour complexité
\newcommand{\ind}{\mathds{1}} % indicatrice




\DeclareMathOperator*{\diag}{\mbox{diag}}
\DeclareMathOperator*{\tr}{\mbox{tr}}
\DeclareMathOperator*{\card}{\mbox{card}}
\DeclareMathOperator*{\cov}{\mbox{cov}}
\DeclareMathOperator*{\sign}{\mbox{sign}}
\DeclareMathOperator*{\var}{\mbox{var}}
%\DeclareMathOperator*{\st}{\mbox{s.t.}}
\DeclareMathOperator*{\rank}{\mbox{rank}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\moyenne}{average}

\DeclareMathOperator*{\Ber}{Ber}
\DeclareMathOperator*{\Beta}{Beta}
\newcommand{\Norm}{{\cal N}}
\DeclareMathOperator*{\sigmoid}{sigmoid}
\DeclareMathOperator*{\logit}{logit}

